Beyond Naturalness: Probing Automated Text-To-Speech Evaluators on Linguistically Grounded Dimensions

Automated Text-to-Speech (TTS) evaluation methods (Mean Opinion Score (MOS) predictors and Audio Large Language Model (Audio-LLM) judges) are expected to reflect human perception, yet it is unclear how well they capture the distinct aspects of speech that listeners actually perceive. We deconstruct "naturalness" into a linguistically grounded annotation schema spanning 10 distinct perceptual dimensions, and use it to construct the first dimension-level meta-evaluation benchmark for TTS, comprising 860 utterances annotated by trained linguist raters. Results from benchmarking four MOS predictors and four Audio-LLM judges reveal that MOS predictors are more sensitive to acoustic signal-level properties at the prosodic and paralinguistic levels, while Audio-LLM judges show selective, prompt-dependent detection that favors word-level errors and does not generalize across all dimensions. Neither class reliably captures a breadth of linguistically structured, human-perceptible speech errors. Our dataset, annotation schema, and evaluation code are publicly released to support more targeted and interpretable TTS evaluation.

==> tables/table4_bootstrap_ci_stacked.tex <==
% Requires: \usepackage{amsmath,booktabs,graphicx}
\begin{table*}[p]
  \centering
  \rotatebox{90}{%
  \begin{minipage}{0.8\textheight}
  \centering
  \footnotesize
  \renewcommand{\arraystretch}{1.20}
  \setlength{\tabcolsep}{3pt}
  \caption{Per-dimension Kendall's $\tau_b$ for \textsc{\audiollm} judges using C2a, C2b, and C3 prompts. Each cell reports the point estimate and its 95\% percentile bootstrap confidence interval in brackets, computed from 5,000 paired item-level resamples.}
  \label{tab:tau_lalm_ci_stacked}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{l | ll | llll | llll}
    \toprule
    \textbf{Model} & \multicolumn{2}{c}{\textbf{Word}} & \multicolumn{4}{c}{\textbf{Prosodic}} & \multicolumn{4}{c}{\textbf{Paralinguistic}} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-7} \cmidrule(lr){8-11}
     & \textbf{Phon.} & \textbf{Lex.} & \textbf{Inton.} & \textbf{Pros.S} & \textbf{Pros.B} & \textbf{Rate} & \textbf{Emo.} & \textbf{Expr.} & \textbf{Spk.} & \textbf{Hum.} \\
    \midrule
    \multicolumn{11}{c}{C2a --- Multi-dimension schema; single holistic score} \\
    \midrule
    Gemini 3 Flash$^\dag$ & \phantom{-}$\underset{\scriptscriptstyle [0.144,\,0.413]}{\mathbf{0.292}^{**}}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.176,\,0.237]}{0.037}$ & \phantom{-}$\underset{\scriptscriptstyle [0.104,\,0.310]}{0.197}$ & \phantom{-}$\underset{\scriptscriptstyle [0.087,\,0.236]}{0.141}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.211,\,0.316]}{0.064}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.170,\,0.170]}{0.000}$ & \phantom{-}$\underset{\scriptscriptstyle [0.137,\,0.416]}{0.264}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.062,\,0.290]}{0.142}$ & \phantom{-}$\underset{\scriptscriptstyle [0.106,\,0.298]}{0.177}$ & \phantom{-}$\underset{\scriptscriptstyle [0.108,\,0.269]}{0.135}$ \\
    Gemini 3 Flash$^\triangle$ & \phantom{-}$\underset{\scriptscriptstyle [0.028,\,0.365]}{\mathbf{0.206}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.162,\,0.468]}{\mathbf{0.327}^{**}}$ & $\underset{\scriptscriptstyle [-0.265,\,-0.097]}{-0.160}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.188,\,0.183]}{0.000}$ & \phantom{-}$\underset{\scriptscriptstyle [0.137,\,0.426]}{\mathbf{0.283}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.011,\,0.288]}{0.172}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.165,\,0.385]}{0.129}$ & \phantom{-}$\underset{\scriptscriptstyle [0.102,\,0.316]}{\mathbf{0.211}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.100,\,0.246]}{0.124}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.252,\,0.247]}{0.000}$ \\
    Gemini 3.5 Flash$^\dag$ & \phantom{-}$\underset{\scriptscriptstyle [0.346,\,0.615]}{\mathbf{0.486}^{***}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.100,\,0.485]}{\mathbf{0.294}^{**}}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.102,\,0.318]}{0.119}$ & \phantom{-}$\underset{\scriptscriptstyle [0.029,\,0.381]}{\mathbf{0.216}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.214,\,0.308]}{0.064}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.172,\,0.172]}{0.000}$ & \phantom{-}$\underset{\scriptscriptstyle [0.143,\,0.633]}{\mathbf{0.396}^{**}}$ & $\underset{\scriptscriptstyle [-0.230,\,0.171]}{-0.031}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.129,\,0.352]}{0.122}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.122,\,0.380]}{0.146}$ \\
    Gemini 3.5 Flash$^\triangle$ & \phantom{-}$\underset{\scriptscriptstyle [0.245,\,0.536]}{\mathbf{0.396}^{***}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.245,\,0.607]}{\mathbf{0.438}^{***}}$ & $\underset{\scriptscriptstyle [-0.258,\,0.173]}{-0.052}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.130,\,0.264]}{0.064}$ & $\underset{\scriptscriptstyle [-0.356,\,0.168]}{-0.104}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.077,\,0.265]}{0.102}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.191,\,0.385]}{0.099}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.029,\,0.354]}{0.170}$ & \phantom{-}$\underset{\scriptscriptstyle [0.068,\,0.496]}{\mathbf{0.296}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.153,\,0.352]}{0.115}$ \\
    Qwen3 Omni$^\dag$ & \phantom{-}$\underset{\scriptscriptstyle [-0.099,\,0.232]}{0.097}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.064,\,0.291]}{0.146}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.175,\,0.252]}{0.052}$ & $\underset{\scriptscriptstyle [-0.245,\,0.100]}{-0.101}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.072,\,0.385]}{0.192}$ & . & . & \phantom{-}$\underset{\scriptscriptstyle [0.097,\,0.284]}{0.182}$ & \phantom{-}$\underset{\scriptscriptstyle [0.228,\,0.623]}{\mathbf{0.435}^{***}}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.231,\,0.230]}{0.000}$ \\
    Qwen3 Omni$^\triangle$ & \phantom{-}$\underset{\scriptscriptstyle [0.094,\,0.288]}{\mathbf{0.194}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.023,\,0.382]}{\mathbf{0.212}^{*}}$ & . & $\underset{\scriptscriptstyle [-0.237,\,-0.087]}{-0.141}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.228,\,0.225]}{0.000}$ & . & . & . & $\underset{\scriptscriptstyle [-0.246,\,-0.100]}{-0.124}$ & \phantom{-}$\underset{\scriptscriptstyle [0.108,\,0.265]}{0.135}$ \\
    Step Audio 2 Mini$^\dag$ & \phantom{-}$\underset{\scriptscriptstyle [-0.184,\,0.187]}{0.000}$ & \phantom{-}$\underset{\scriptscriptstyle [0.099,\,0.292]}{0.186}$ & . & $\underset{\scriptscriptstyle [-0.245,\,0.101]}{-0.101}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.262,\,0.252]}{0.000}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.146,\,0.148]}{0.000}$ & \phantom{-}$\underset{\scriptscriptstyle [0.125,\,0.368]}{0.213}$ & $\underset{\scriptscriptstyle [-0.242,\,-0.091]}{-0.147}$ & \phantom{-}$\underset{\scriptscriptstyle [0.188,\,0.613]}{\mathbf{0.413}^{***}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.104,\,0.275]}{0.135}$ \\
    Step Audio 2 Mini$^\triangle$ & \phantom{-}$\underset{\scriptscriptstyle [-0.149,\,0.227]}{0.041}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.208,\,0.210]}{0.000}$ & \phantom{-}$\underset{\scriptscriptstyle [0.097,\,0.271]}{0.160}$ & $\underset{\scriptscriptstyle [-0.235,\,0.144]}{-0.039}$ & $\underset{\scriptscriptstyle [-0.374,\,0.151]}{-0.111}$ & $\underset{\scriptscriptstyle [-0.379,\,-0.049]}{\mathbf{-0.221}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.296,\,0.280]}{0.000}$ & $\underset{\scriptscriptstyle [-0.357,\,0.031]}{-0.165}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.180,\,0.303]}{0.061}$ & $\underset{\scriptscriptstyle [-0.400,\,0.119]}{-0.153}$ \\
    \midrule
    \multicolumn{11}{c}{C2b --- Multi-dimension schema; one score per dimension} \\
    \midrule
    Gemini 3 Flash$^\dag$ & \phantom{-}$\underset{\scriptscriptstyle [0.290,\,0.504]}{\mathbf{0.397}^{***}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.089,\,0.208]}{0.106}$ & . & . & \phantom{-}$\underset{\scriptscriptstyle [0.114,\,0.331]}{0.196}$ & . & \phantom{-}$\underset{\scriptscriptstyle [0.114,\,0.301]}{0.149}$ & \phantom{-}$\underset{\scriptscriptstyle [0.087,\,0.202]}{0.104}$ & . & . \\
    Gemini 3 Flash$^\triangle$ & \phantom{-}$\underset{\scriptscriptstyle [0.096,\,0.289]}{\mathbf{0.194}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.097,\,0.286]}{0.186}$ & . & . & . & . & . & \phantom{-}$\underset{\scriptscriptstyle [0.087,\,0.202]}{0.104}$ & . & . \\
    Gemini 3.5 Flash$^\dag$ & \phantom{-}$\underset{\scriptscriptstyle [0.405,\,0.624]}{\mathbf{0.514}^{***}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.166,\,0.401]}{\mathbf{0.290}^{**}}$ & . & . & \phantom{-}$\underset{\scriptscriptstyle [0.110,\,0.282]}{0.137}$ & \phantom{-}$\underset{\scriptscriptstyle [0.080,\,0.208]}{0.126}$ & \phantom{-}$\underset{\scriptscriptstyle [0.149,\,0.462]}{\mathbf{0.309}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.102,\,0.317]}{\mathbf{0.211}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.106,\,0.298]}{0.177}$ & \phantom{-}$\underset{\scriptscriptstyle [0.108,\,0.268]}{0.135}$ \\
    Gemini 3.5 Flash$^\triangle$ & \phantom{-}$\underset{\scriptscriptstyle [0.042,\,0.340]}{\mathbf{0.210}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.087,\,0.206]}{0.106}$ & \phantom{-}$\underset{\scriptscriptstyle [0.094,\,0.224]}{0.113}$ & . & \phantom{-}$\underset{\scriptscriptstyle [0.110,\,0.271]}{0.137}$ & \phantom{-}$\underset{\scriptscriptstyle [0.076,\,0.173]}{0.089}$ & \phantom{-}$\underset{\scriptscriptstyle [0.114,\,0.301]}{0.149}$ & \phantom{-}$\underset{\scriptscriptstyle [0.091,\,0.250]}{0.147}$ & \phantom{-}$\underset{\scriptscriptstyle [0.113,\,0.336]}{0.218}$ & \phantom{-}$\underset{\scriptscriptstyle [0.108,\,0.265]}{0.135}$ \\
    Qwen3 Omni$^\dag$ & . & . & . & . & . & . & . & . & . & . \\
    Qwen3 Omni$^\triangle$ & . & . & . & . & . & . & . & $\underset{\scriptscriptstyle [-0.206,\,-0.087]}{-0.104}$ & . & . \\
    Step Audio 2 Mini$^\dag$ & . & . & . & . & . & . & . & . & . & . \\
    Step Audio 2 Mini$^\triangle$ & . & . & \phantom{-}$\underset{\scriptscriptstyle [-0.126,\,0.285]}{0.095}$ & . & . & . & \phantom{-}$\underset{\scriptscriptstyle [0.120,\,0.306]}{0.149}$ & . & . & . \\
    \midrule
    \multicolumn{11}{c}{C3 --- Single-dimension focus; one dimension at a time} \\
    \midrule
    Gemini 3 Flash$^\dag$ & \phantom{-}$\underset{\scriptscriptstyle [0.258,\,0.469]}{\mathbf{0.366}^{***}}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.178,\,0.185]}{0.000}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.142,\,0.286]}{0.083}$ & . & \phantom{-}$\underset{\scriptscriptstyle [0.166,\,0.465]}{\mathbf{0.319}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.076,\,0.171]}{0.089}$ & \phantom{-}$\underset{\scriptscriptstyle [0.125,\,0.365]}{0.213}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.144,\,0.216]}{0.061}$ & . & . \\
    Gemini 3 Flash$^\triangle$ & \phantom{-}$\underset{\scriptscriptstyle [0.155,\,0.363]}{\mathbf{0.261}^{**}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.147,\,0.378]}{\mathbf{0.267}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.218,\,0.216]}{0.000}$ & . & \phantom{-}$\underset{\scriptscriptstyle [-0.210,\,0.308]}{0.055}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.156,\,0.198]}{0.021}$ & \phantom{-}$\underset{\scriptscriptstyle [0.125,\,0.355]}{0.213}$ & $\underset{\scriptscriptstyle [-0.252,\,0.152]}{-0.054}$ & . & \phantom{-}$\underset{\scriptscriptstyle [0.104,\,0.268]}{0.135}$ \\
    Gemini 3.5 Flash$^\dag$ & \phantom{-}$\underset{\scriptscriptstyle [0.250,\,0.461]}{\mathbf{0.355}^{***}}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.019,\,0.326]}{0.178}$ & . & . & \phantom{-}$\underset{\scriptscriptstyle [0.128,\,0.384]}{0.243}$ & \phantom{-}$\underset{\scriptscriptstyle [0.015,\,0.323]}{\mathbf{0.181}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.288,\,0.628]}{\mathbf{0.459}^{**}}$ & $\underset{\scriptscriptstyle [-0.256,\,0.144]}{-0.060}$ & \phantom{-}$\underset{\scriptscriptstyle [0.152,\,0.414]}{\mathbf{0.286}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.104,\,0.275]}{0.135}$ \\
    Gemini 3.5 Flash$^\triangle$ & \phantom{-}$\underset{\scriptscriptstyle [0.094,\,0.286]}{\mathbf{0.194}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.039,\,0.351]}{0.170}$ & $\underset{\scriptscriptstyle [-0.318,\,0.071]}{-0.155}$ & \phantom{-}$\underset{\scriptscriptstyle [0.085,\,0.198]}{0.100}$ & \phantom{-}$\underset{\scriptscriptstyle [0.029,\,0.465]}{\mathbf{0.276}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.062,\,0.381]}{\mathbf{0.232}^{**}}$ & \phantom{-}$\underset{\scriptscriptstyle [0.041,\,0.515]}{\mathbf{0.303}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.165,\,0.245]}{0.043}$ & \phantom{-}$\underset{\scriptscriptstyle [0.113,\,0.344]}{0.218}$ & $\underset{\scriptscriptstyle [-0.275,\,-0.108]}{-0.135}$ \\
    Qwen3 Omni$^\dag$ & . & . & . & . & \phantom{-}$\underset{\scriptscriptstyle [0.110,\,0.282]}{0.137}$ & $\underset{\scriptscriptstyle [-0.349,\,-0.013]}{\mathbf{-0.184}^{*}}$ & . & \phantom{-}$\underset{\scriptscriptstyle [-0.185,\,0.225]}{0.026}$ & . & \phantom{-}$\underset{\scriptscriptstyle [-0.106,\,0.416]}{0.165}$ \\
    Qwen3 Omni$^\triangle$ & \phantom{-}$\underset{\scriptscriptstyle [0.084,\,0.226]}{0.136}$ & \phantom{-}$\underset{\scriptscriptstyle [0.119,\,0.354]}{\mathbf{0.243}^{*}}$ & . & . & \phantom{-}$\underset{\scriptscriptstyle [0.034,\,0.552]}{\mathbf{0.298}^{*}}$ & \phantom{-}$\underset{\scriptscriptstyle [-0.127,\,0.224]}{0.050}$ & $\underset{\scriptscriptstyle [-0.292,\,-0.114]}{-0.149}$ & $\underset{\scriptscriptstyle [-0.406,\,-0.015]}{\mathbf{-0.214}^{*}}$ & . & \phantom{-}$\underset{\scriptscriptstyle [-0.135,\,0.345]}{0.139}$ \\
    Step Audio 2 Mini$^\dag$ & . & . & . & . & . & . & . & \phantom{-}$\underset{\scriptscriptstyle [0.087,\,0.202]}{0.104}$ & . & \phantom{-}$\underset{\scriptscriptstyle [-0.269,\,0.267]}{0.000}$ \\
    Step Audio 2 Mini$^\triangle$ & . & $\underset{\scriptscriptstyle [-0.215,\,-0.090]}{-0.108}$ & . & \phantom{-}$\underset{\scriptscriptstyle [0.085,\,0.198]}{0.100}$ & . & . & . & \phantom{-}$\underset{\scriptscriptstyle [-0.130,\,0.265]}{0.069}$ & . & \phantom{-}$\underset{\scriptscriptstyle [-0.220,\,0.296]}{0.038}$ \\
    \bottomrule
  \end{tabular}%
  }
  \vspace{4pt}
  \parbox{\linewidth}{\footnotesize
    \textbf{Columns:} Phon.\,=\,Phonetic Accuracy; Lex.\,=\,Lexical Stress; Inton.\,=\,Intonation; Pros.S\,=\,Prosodic Stress; Pros.B\,=\,Prosodic Boundary; Rate\,=\,Speech Rate; Emo.\,=\,Emotional Appropriateness; Expr.\,=\,Expressiveness; Spk.\,=\,Speaker Identity; Hum.\,=\,Human Plausibility. \textbf{Transcript:} $^\dag$\,=\,with transcript; $^\triangle$\,=\,without transcript. \textbf{Bold} = significant ($p<.05$). $^{*}p<.05$, $^{**}p<.01$, $^{***}p<.001$ (two-sided). A dot indicates undefined $\tau_b$ because the model produced a constant prediction; no confidence interval is reported for undefined cells.}
  \end{minipage}%
  }
\end{table*}

